A fast solver for the spatially homogeneous electron Boltzmann equation

We present a numerical method for the velocity-space, spatially homogeneous, collisional Boltzmann equation for electron transport in low-temperature plasma (LTP) conditions. Modeling LTP plasmas is useful in many applications, including advanced manufacturing, material processing, semiconductor processing, and hypersonics, to name a few. Most state-of-the-art methods for electron kinetics are based on Monte-Carlo sampling for collisions combined with Lagrangian particle-in-cell methods. We discuss an Eulerian solver that approximates the electron velocity distribution function using spherical harmonics (angular components) and B-splines (energy component). Our solver supports electron-heavy elastic and inelastic binary collisions, electron-electron Coulomb interactions, steady-state and transient dynamics, and an arbitrary nmber of angular terms in the electron distribution function. We report convergence results and compare our solver to two other codes: an in-house particle Monte-Carlo ethod; and Bolsig+, a state-of-the-art Eulerian solver for electron transport in LTPs. Furthermore, we use our solver to study the relaxation time scales of the higher-order anisotropic correction terms. Our code is open-source and provides an interface that allows coupling to multiphysics simulations of low-temperature plasmas.

==> bolsig_comparison.tex <==
\section{BOLSIG Comparison}



==> boltzmann_eqn.tex <==
\section{Boltzmann}

0D3V Boltzmann equation and discussion

\begin{equation}
    \frac{\partial f_e}{\partial t} + \frac{-eE}{m_k}\cdot \nabla_c f_e = C[f]
\end{equation}

Discussion

\subsection{Physics of Coulombic collisions}

Coulomb collisions are binary elastic collisions between charged particles. In the case of ionized plasmas, these can be electron-electron, electron-ion, or ion-ion collisions. The work presented in limits discussion to electron-electron collisions. Higher electron densities lead to higher Coulombic collison rates. These collisions smoothen the distribution functions and push them closer to those of a Maxwellian

==> dg.tex <==
\subsection{Discontinuous Galerkin discretization}
\label{subsec:dg_formulation}

%\begin{figure}[!tbhp]
%    \centering
%    \begin{tikzpicture}
%        \draw[thick, black] (0,0) -- (8,0);
%        \draw[thick, black] (0,-0.2) --node[below]{$v_0$} (0,0.2);
%        \draw[thick, black] (4,-0.2) --node[below]{$v_1$} (4,0.2);
%        \draw[thick, black] (8,-0.2) --node[below]{$v_2$} (8,0.2);
%        \node at (2,-0.5) {$\Omega_0$};
%        \node at (6,-0.5) {$\Omega_1$};
%    \end{tikzpicture}
%\caption{An example of two discontinuous domains $\Omega_0$ and $\Omega_1$ in the radial coordinate. The discontinuity points are placed at energy threshold values for different inelastic collisions.} \label{fig:dg_domains}
%\end{figure}
Electron-heavy collision cross-section data can be non-smooth functions of energy. For example, ionization collisions occur if and only if the electron energy is greater than ionization threshold energy $\epsilon_0$ (i.e., $\epsilon_0$ = 15.76 eV for Argon). There are two key challenges for continuous radial basis representation for the distribution function. 1). Non-smooth cross-section data triggers non-smooth distribution functions. 2). Up-winded numerical scheme is required to handle cases with strong advection. There are several approaches to resolving the above challenges. They can be summarized as follows.  1). Add a diffusive term (i.e., numerical stabilization or derived from the problem itself) 2). Discontinuous basis representation of $f$ where discontinuities are placed exactly at the reaction threshold values. The Coulomb collision operator serves as a diffusion operator that can help to remove the numerical instabilities discussed above. Hence, we consider discontinuous Galerkin derivation in the absence of the Coulomb collisions. Therefore, we use the continuous Galerkin approach in the presence of Coulomb interactions while the discontinuous Galerkin method is used in the absence of Coulomb interactions. In this section we summarize the discretization of advection and electron-heavy collision operators using discontinuous Galerkin approach. 

We consider two adjacent discontinuous domains $\Omega_0$ and $\Omega_1$. Let $f(\vect{v}) = \sum_{lm} f_{lm}\of{v} Y_{lm}\of{\vtheta,\vphi}$. By substituting the above in \Cref{eq:adv_term}, we can derive equations \Cref{eq:adv_term_dg} and \Cref{eq:adv_term_dg_ws}. 
\begin{align}
\vect{E}\cdot \nabla_{\vect{v}} f &= E 
\sum_{lm} 
\Bigg(
\left( A_M\of{l,m} \frac{d}{d\vr}f_{lm}\of{\vr} 
+ A_D\of{l,m} \frac{1}{\vr}f_{lm}\of{\vr} \right)
Y_{(l-1)m}\of{\vtheta,\vphi} 
\nonumber\\
&+
\left( B_M\of{l,m} \frac{d}{d\vr}f_{lm}\of{\vr} 
+ B_D\of{l,m} \frac{1}{\vr}f_{lm}\of{\vr} \right)
Y_{(l+1)m}\of{\vtheta,\vphi} 
\Bigg) \label{eq:adv_term_dg} \\
\myint \vect{E}\cdot \nabla_{\vect{v}} f Y_{qs}\of{\theta,\phi} \diff{\vomega}
&= E 
\Bigg(
\left( A_M\of{q+1,s} \frac{d}{d\vr} f_{q+1,s} \of{\vr} 
+ A_D\of{q+1,s} \frac{1}{\vr} f_{q+1,s} \of{\vr} \right)
\nonumber \\
&+ \left( B_M\of{q-1,s} \frac{d}{d\vr} f_{q-1,s} \of{\vr} 
+ B_D\of{q-1,s} \frac{1}{\vr} f_{q-1,s} \of{\vr} \right)
\Bigg) \label{eq:adv_term_dg_ws}
\end{align}
For the collision operator, we start with the simplified operator under azimuthal symmetry and isotropic scattering assumptions. Under the above assumptions we can write the weak form of the collision operator projected onto the spherical basis as in \Cref{eq:en_coll_op_sph}.
\begin{align}
	C^{q0}_{l0}  = n_0 \myint_{\reals^+} v^3 \sigma\of{\varepsilon} f_{l}\of{v} \delta_{ql} \of{\phi\of{v^\prime}\delta_{q0} - \phi\of{v}} \diff{v} \text{ where } v^\prime = v^{post}\of{v} \label{eq:en_coll_op_sph}
\end{align} For inelastic collisions with energy threshold $\epsilon_0$ (in eV), we can write the collision operator discretization for domain $\Omega_0$ as in \Cref{eq:dg_coll_op_inelastic} where energy $\epsilon$ (in eV) can be written as $\epsilon=\of{\frac{v}{\gamma}}^2$ with $\gamma=\sqrt{2q_e/m_e}$.
\begin{equation}
    [C_{en}^{\Omega_0}]^{q0}_{l0} = 
    \begin{cases}
        \int_{v_0 + \sqrt{\epsilon_0}\gamma}^{v1 + \sqrt{\epsilon_0}\gamma} v^3 \sigma f_{l0}\of{v} \phi^{(\Omega_0)}\of{v^\prime} dv - \int_{v_0}^{v_1} v^3 \sigma f_{l0}^{(\Omega_0)}\of{v} \phi^{(\Omega_0)}\of{v} dv & (q,l)=(0,0)\\
        - \int_{v_0}^{v_1} v^3 \sigma f_{l0}^{(\Omega_0)}\of{v} \phi^{(\Omega_0)}\of{v} dv & (q,l) > (0,0)\\
        0 & q!=l            
    \end{cases}
    \label{eq:dg_coll_op_inelastic}
\end{equation}
For elastic collisions, the mode (q,l)=(0,0) needs to be treated properly to couple the discontinuous domains. The above is because the energy loss in the collision process is quite small (i.e., for Argon $\approx 10^{-5}$) and requires a quadrature grid with a resolution smaller than the energy loss to capture it by \Cref{eq:dg_coll_op_inelastic}. To overcome the above challenge, we analytically split the integrals, such that discontinuous domains are coupled as in \Cref{eq:dg_coll_op_elastic} where $v^\prime = \sqrt{(1-\mu)}v$ and $\mu=m_e/M$ with $M$ denoting the mass of the heavy particle. 
\begin{multline}
    [C_{en}^{\Omega_0}]^{00}_{00} =
    \int_{v_0/\sqrt{1-\mu}}^{v_1} v^3 \sigma f_{l0}^{(\Omega_0)}\of{v} \phi^{(\Omega_0)}\of{v^\prime} dv 
    + \int_{v_1}^{v_1/\sqrt{1-\mu}} v^3 \sigma f_{l0}^{(\Omega_1)}\of{v} \phi^{(\Omega_0)}\of{v^\prime}dv \\
    -\int_{v_0}^{v_0/\sqrt{1-\mu}} v^3 \sigma f_{l0}^{(\Omega_0)}\of{v} \phi^{(\Omega_0)}\of{v} dv
    -\int_{v_0/\sqrt{1-\mu}}^{v_1}v^3 \sigma f_{l0}^{(\Omega_0)}\of{v} \phi^{(\Omega_0)}\of{v} dv 
    \label{eq:dg_coll_op_elastic}
\end{multline}
We can write \Cref{eq:bte} projected onto spherical harmonics as in \Cref{eq:dg_bte} where $A^{q0}_{l0}$ and $B^{q0}_{l0}$ are constant coefficient matrices determined by the coefficients in \Cref{eq:adv_term_dg_ws}.  
\begin{align}
    \partial_t f_{q0}  - E A^{q0}_{l0} \partial_{v} f_{l0} - E B^{q0}_{l0} \frac{1}{v} f_{l0} = [C_{en}]^{q0}_{l0} f_{l0} \label{eq:dg_bte}
\end{align} By looking at \Cref{eq:adv_term_dg_ws} that the advection operator couples each $l$ mode to $l+1$ and $l-1$ modes. To enable up-winding, we solve the diagonalized system, where $A^{q0}_{l0} = W \Lambda W^T$ with $y_{q0}=[W^T]^{q0}_{l0} f_{l0}$. The diagonalized system can be written as \Cref{eq:dg_bte_diagonalized}. With \Cref{eq:dg_bte_diagonalized} system substituting $f_{l0}\of{v} = \sum_{k} f_{kl0} \phi_{k}\of{v}$ and using integration by parts for the radial coordinate derivative term, we can derive the complete weak form for the diagonalized system.
\begin{align}
\partial_t y_{q0}  - E \Lambda \partial_{v} y_{l0} - E W^T B^{q0}_{l0} \frac{1}{v} W y_{l0} = W^T [C_{en}]^{q0}_{l0} W y_{l0} \label{eq:dg_bte_diagonalized}
\end{align}

==> dsmc_selfconvergence.tex <==
\section{Self-Convergence: Particle Code}
aaa

\subsection{Convergence by Num Particles}

aaa
\subsection{Convergence by Timestep size}
aaa

==> experiments.tex <==


%We perform 0D-3V simulations of electrons in which a 1-D constant electric field is applied to the system. The background neutral Argon density is assumed to be constant. When Coulombic collisions are considered, the electron density is specified.


%\input{pde_results.tex}



% DSMC stuff. 
% \input{measurables}
% \input{fmodes}
% \input{transients}
% \input{dsmc_selfconvergence}




==> fmodes.tex <==
\subsection{F Mode Comparison}

We now compare the F modes between the particle and determinstic codes along with a comparison to Bolsig. In the case of the deterministic and Bolsig codes, these F modes are unknowns that are directly solved for. In each of these cases, only a finite number of F modes can be solved for. Bolsig uses a two-term approximation and only solves for $F_0$ and $F_1$. Our deterministic code has the functionality to solve up to $l=6$ (or whatever is true). The particle code, however, does not consider these F modes as unkowns, but rather they are computed in a post-processing step. In this way, the particle code can be seen as more "exact" in the sense that there is no term approximation or cutoff. The details of the calculations of the F modes using the particle code are provided in the appendix. Below, we show some example cases of $F$ modes something.



We note that the particle code often poorly captures the $F_l$ modes for high values of $l$. As detailed in the appendix, the functions that we try to capture with integration become increasingly oscillatory as $l$ grows. Monte Carlo integration struggles to accurately converge these integrals, as it has $O(\sqrt{N})$ scaling.

==> measurables.tex <==
\subsection{Measurable errors: Particle code}

Using both the deterministic and the particle codes, we calculate the steady state values for temperature, rate coefficients, and mobility. We report the relative errors in measured steady state quantities compared to results given by Bolsig, the industry standard for such problems.
We report the relative errors to Bolsig of our code 
\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
     &  $10^{-1}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-5}$ & $10^{-6}$ \\
    \hline
    \hline
    1Td & $5.6\times 10^{-4}$ & $2.4\times 10^{-3}$ & $1.5\times 10^{-3}$ & $1.7\times 10^{-3}$ & $4.0\times 10^{-3}$ & $2.1\times 10^{-3}$ \\
    \hline
    5Td & $1.8\times 10^{-3}$ & $1.0\times 10^{-3}$ & $1.0\times 10^{-3}$ & $3.3\times 10^{-4}$ & $3.2 \times 10^{-5}$ & $1.9 \times 10^{-4}$ \\
    \hline
    20Td & $2.1\times 10^{-3}$ & $1.5\times 10^{-3}$ & $6.9\times 10^{-4}$ & $1.6\times 10^{-3}$ & $8.9\times 10^{-4}$ & $3.1\times 10^{-4}$ \\
    \hline
    100Td & $2.5\times 10^{-3}$ & $1.3\times 10^{-3}$ & $5.9\times 10^{-3}$ & $4.1\times 10^{-3}$ & $3.5\times 10^{-3}$ & $3.2\times 10^{-3}$ \\
    \hline
\end{tabular}
\caption{Temperature Errors (Particle code)}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
     &  $10^{-1}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-5}$ & $10^{-6}$ \\
    \hline
    \hline
    1Td & $5.8 \times 10^{-3}$ & $8.7 \times 10^{-3}$ & $6.2 \times 10^{-3}$ & $3.5 \times 10^{-3}$ & $1.2 \times 10^{-2}$ & $7.8 \times 10^{-3}$ \\
    \hline
    5Td & $3.4 \times 10^{-3}$ & $4.8 \times 10^{-3}$ & $5.9 \times 10^{-3}$ & $8.2 \times 10^{-3}$ & $7.1 \times 10^{-3}$ & $7.8 \times 10^{-3}$ \\
    \hline
   20Td & $3.3\times 10^{-3}$ & $5.4\times 10^{-3}$ & $8.2\times 10^{-3}$ & $9.8\times 10^{-3}$ & $9.8\times 10^{-3}$ & $8.3\times 10^{-3}$ \\
    \hline
    100Td & $5.5\times 10^{-3}$ & $1.0\times 10^{-2}$ & $1.5\times 10^{-2}$ & $1.3\times 10^{-2}$ & $1.2\times 10^{-2}$ & $1.1\times 10^{-2}$ \\
    \hline
\end{tabular}
\caption{Elastic Rate Coefficient Errors (Particle code)}
\end{table}

\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
     &  $10^{-1}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-5}$ & $10^{-6}$ \\
    \hline
    \hline
    1Td & $3.2 \times 10^{-2}$ & $1.4 \times 10^{-2}$ & $7.6 \times 10^{-3}$ & $2.7 \times 10^{-2}$ & $7.9 \times 10^{-3}$ & - \\
    \hline
    5Td & $3.0 \times 10^{-4}$ & $4.7 \times 10^{-3}$ & $6.6 \times 10^{-3}$ & $9.6 \times 10^{-3}$ & $8.1 \times 10^{-3}$ & $1.9 \times 10^{-3}$ \\
    \hline
    20Td & $1.1\times 10^{-2}$ & $5.7\times 10^{-3}$ & $1.1\times 10^{-2}$ & $7.3\times 10^{-3}$ & $9.1\times 10^{-3}$ & $4.8\times 10^{-3}$ \\
    \hline
    100Td & $5.6\times 10^{-3}$ & $2.0\times 10^{-2}$ & $2.4\times 10^{-2}$ & $1.5\times 10^{-2}$ & $1.4\times 10^{-2}$ & $8.3\times 10^{-3}$ \\
    \hline
\end{tabular}
\caption{Ionization Rate Coefficient Errors (Particle code)}
\end{table}


\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
     &  $10^{-1}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-5}$ & $10^{-6}$ \\
    \hline
    \hline
    1Td & $6.7 \times 10^{-3}$ & $5.0 \times 10^{-3}$ & $3.2 \times 10^{-3}$ & $2.3 \times 10^{-3}$ & $3.4 \times 10^{-4}$ & $4.8 \times 10^{-3}$ \\
    \hline
    5Td & $8.8\times 10^{-3}$ & $4.2 \times 10^{-3}$ & $5.9 \times 10^{-4}$ & $4.1 \times 10^{-3}$ & $1.6 \times 10^{-2}$ & $1.9 \times 10^{-3}$ \\
    \hline
    20Td & $9.6\times 10^{-3}$ & $2.1\times 10^{-3}$ & $4.7\times 10^{-3}$ & $4.0\times 10^{-3}$ & $3.2\times 10^{-3}$ & $3.9\times 10^{-3}$ \\
    \hline
    100Td & $2.6\times 10^{-3}$ & $1.4\times 10^{-2}$ & $1.8\times 10^{-2}$ & $7.9\times 10^{-2}$ & $1.1\times 10^{-1}$ & $5.1\times 10^{-3}$ \\
    \hline
\end{tabular}
\caption{Mobility Errors (Particle code)}
\end{table}

==> pde_selfconvergence.tex <==
\section{Self-Convergence}
aaa
\subsection{Convergence by A}
aaa
\subsection{Convergence by B}
aaa

==> relatedwork.tex <==
There exist several state-of-the-art codes to compute deterministic solutions for the spatially homogeneous Boltzmann equation. \textsc{ELENDIF}~\cite{morgan1990elendif} uses two-term approximation $f(v,\vtheta) = f_0(v) + f_1(v)\cos(\vtheta)$ for the electron distribution function with capabilities for inelastic, electron-electron and several other collisional processes. The well-known \bolsig~\cite{hagelaar2005solving,hagelaar2015coulomb}  uses the same two-term approximation with exponential finite differences. \text{ZDPlasKin}~\cite{pancheshnyi2008zdplaskin} is another tool for plasma kinetic simulations where \bolsig~code is used as the underlying Boltzmann solver. To the best of our knowledge, existing deterministic solvers are limited by the two-term approximation and mostly use finite differences approximations as the main discretization approach. There have been several noticeable work~\cite{gamba2018galerkin, alekseenko2014deterministic} on using Galerkin approach for solving the Boltzmann equation. The above works mainly rely on the analytical cross-section approximations with no support for Coulomb interactions. In~\cite{gamba2018galerkin} proposes global polynomial approximations for the radial coordinate direction, while we found global approximations does not work well with non-smooth tabulated cross-sections. Direct simulation Monte Carlo (DSMC)~\cite{bird1994molecular} is another state-of-the-art approach for solving the Boltzmann equation. There exists several DSMC codes~\cite{scanlon2010open, zabelok2015adaptive, frezzotti2011solving, oblapenko2020velocity, bartel2003modelling, lymberopoulos1994stochastic} in the literature. In this work we use our own DSMC code which is based on the null collisional method~\cite{vahedi1995monte} and~\cite{PhysRevE.55.4642} for Coulomb interactions. 



%\begin{itemize}
%    \item Deterministic approach
%    \item https://arxiv.org/pdf/1301.1099.pdf - We present a new deterministic approach for the solution of the Boltzmann kinetic equation based on nodal
%    discontinuous Galerkin (DG) discretizations in velocity space. In the new approach the collision operator
%    has the form of a bilinear operator with pre-computed kernel; its evaluation requires O(n5) operations at
%    every point of the phase space where n is the number of degrees of freedom in one velocity dimension. The
%    method is generalized to any molecular potential. Results of numerical simulations are presented for the
%    problem of spatially homogeneous relaxation for the hard spheres potential. Comparison with the method
%    of Direct Simulation Monte Carlo (DSMC) showed excellent agreement.
%    
%    \item https://web.ma.utexas.edu/users/gamba/papers/GR-JCP2018.pdf - No advection, only with elastic collisions, no tabulated cross-section data. 
%    In this work, we propose a new Galerkin–Petrov method for the numerical solution
%    of the classical spatially homogeneous Boltzmann equation. This method is based on
%    an approximation of the distribution function by associated Laguerre polynomials and
%    spherical harmonics and test in a variational manner with globally defined three-
%    dimensional polynomials. A numerical realisation of the algorithm is presented. The
%    algorithmic developments are illustrated with the help of several numerical tests.
%    
%    \item https://par.nsf.gov/servlets/purl/10159570 - The Boltzmann equation, a six-dimensional integro-differential equation, governs the fluid flow behavior at molecular level for a wide range of physical phenomena, including shocks, turbulence, diffusion, and non-equilibrium chemistry which are
%    beyond the reach of continuum fluid flow modelling based on the Navier-Stokes equations. Despite Boltzmann equation’s wide
%    applicability, its deterministic solution presents a huge computational challenge, and has been so far tractable only in simplified
%    forms. We implement the Discontinuous Galerkin Fast Spectral (DGFS) method (Jaiswal, Alexeenko, and Hu 2019 [1]) for solving
%    the full Boltzmann equation on streaming multi-processors. The proposed method is flexible and robust allowing: a) arbitrary un-
%    structured geometries, b) control of spatial accuracy using high-order polynomial approximation without compromising simulation
%    stability, c) exponential error convergence (spectral accuracy) in velocity space, and d) compact nature of DG as well as collision
%    operator thus minimizing communication and maximizing parallel efficiency. The DG operators (for instance gradient, curl, etc),
%    as well as the collision operator is applied in an element-local way, with flux-based element-to-element coupling. It is this locality
%    that equips DGFS with strong parallel performance on streaming multi-processors. In the present work, we describe, devise and
%    implement DGFS for General-Purpose Graphics Processing Units (GP-GPU). We consider the simulations of 0D spatially homoge-
%    neous, and rarefied 1D Fourier heat transfer. A speedup of approximately 10–100x, and parallel efficiency of 0.95 is demonstrated
%    on multi-CPU/multi-GPU architectures. It is this speedup that now allows researchers to solve problems within a day that would
%    otherwise take months on traditional CPUs. The key optimizations and techniques used to achieve these GPU performance results
%    have been highlighted.
%    \item 
%    \begin{itemize}
%        \item Bolsig and Bolsig+
%        \item ELENDIF - ELENDIF calculates the time evolution of the electron energy distribution function in a mixture of partially ionized gases
%        with or without an applied electric field. The code can treat inelastic and superelastic processes, electron—electron and
%        electron—ion collisions, photon—electron (free—free) processes, attachment and recombination, ionization including a distribu-
%        tion of secondary electrons, and an external source of electrons (e.g. an electron beam). The code also computes the mean
%        electron energy, drift velocity, diffusion coefficient, rate coefficients and energy flow rates for the processes being included in
%        the calculation
%        \item ZDPlasKin - time evolution with Bolsig
%    \end{itemize}
%    \item DSMC approach
%    \begin{itemize}
%        \item 
%    \end{itemize}
%\end{itemize}


==> transients.tex <==
\subsection{Transient Solutions}

The final experiment we consider looks at the rate of convergence of the measurables as well as the distribution function when we initialize with an anisotropic distribution. We can study this as a function of electron density, electric field, and degree of anisotropy in the initial condition.
